Towards Practical Multi-Object Manipulation using Relational Reinforcement Learning

Learning robotic manipulation tasks using reinforcement learning with sparse rewards is currently impractical due to the outrageous data requirements. Many practical tasks require manipulation of multiple objects, and the complexity of such tasks increases with the number of objects. Learning from a curriculum of increasingly complex tasks appears to be a natural solution, but unfortunately, does not work for many scenarios. We hypothesize that the inability of the state-of-the-art algorithms to effectively utilize a task curriculum stems from the absence of inductive biases for transferring knowledge from simpler to complex tasks. We show that graph-based relational architectures overcome this limitation and enable learning of complex tasks when provided with a simple curriculum of tasks with increasing numbers of objects. We demonstrate the utility of our framework on a simulated block stacking task. Starting from scratch, our agent learns to stack six blocks into a tower. Despite using step-wise sparse rewards, our method is orders of magnitude more data-efficient and outperforms the existing state-of-the-art method that utilizes human demonstrations. Furthermore, the learned policy exhibits zero-shot generalization, successfully stacking blocks into taller towers and previously unseen configurations such as pyramids, without any further training.

==> old.tex <==
% \begin{equation}
% \label{eq:multigoalobjective}
% % \mathbb{E}_{g \sim \rho(g|n)} [\sum_{i=t}^T \mathop{\mathbb{E}}_{(s_i, a_i, s_{i+1}) \sim \rho_\pi}[\gamma^{(i-t)} r_i']] \\
% \max_\pi \sum_{n=1}^N \mathbb{E}_{s_g\sim \rho(s_g|n), a \sim \pi, s \sim \mathcal{T}} [\sum_{i=t}^T \gamma^{(t-i)} r(s_t, a_t, s_g^n)]
% \end{equation} 
% where $n$ is the task id and goal $s_g$ is sampled from a goal distribution $\rho(s_g|n)$.

%While it is possible to learn a goal-conditioned policy using on-policy methods~\cite{schulman2015trust,mnih2016asynchronous}, 
%\subsection{Problem Description} 
%We desire a policy that maximizes reward over a target task distribution $\rho(t | \tau_F)$. 
%To make use of a curriculum, we train on a sequence of task distributions $\rho(t | \tau)$ indexed by training stage 1 $\leq \tau \leq \tau_F$. Each task $t$ defines a goal sampling distribution $\rho(g | t)$. Our objective is to maximize performance of our policy over the final task distribution $\rho(t | \tau_F)$. Taking the expectation of (\ref{eq:multigoalobjective}) over $\rho(t|\tau_F)$, we arrive at the maximization objective for the final stage

%\begin{equation}
%\mathbb{E}_{t \sim \rho(t | \tau_F)} [\mathbb{E}_{g \sim \rho(g|t)} [\sum_{i=t}^T \mathop{\mathbb{E}}_{(s_i, a_i, s_{i+1}) \sim \rho_\pi}[\gamma^{(i-t)} r_i']]]
%\end{equation} 



%The tasks we consider have compositional structure that is well-represented by a graph with an edge function shared by every node. For our object manipulation task, we view the physical scene of the environment as such a graph, a formulation that has been explored previously for predicting the physical evolution of a scene over time and for model-based control \cite{interactionnet16, chang2016compositional}. In this formulation, node features are representative of local object properties such as the object's position and velocity, and edges represent interactions between objects (such as collision forces) that are useful for prediction.

%One practical solution to learn from less data is to reward the agent for achieving intermediate sub-goals. However, this also means that an agent can obtain a high reward by only completing these sub-goals without solving the overall task. Such a non-intuitive and complex relationship between rewards and the learned behavior is the core challenge of reward-design. The alternative is to make use of \textit{sparse rewards}: i.e., provide the agent with positive reinforcement only when it completes the overall task. While sparse rewards are relatively easy to define, training with sparse rewards drastically complicates the challenge of credit-assignment and consequently exacerbates the data efficiency problem. 

%How can we enable the transfer of strategies between highly related tasks?
%To better appreciate the challenges in transferring strategies across tasks,  consider the example task of stacking blocks into a tower. Learning to stack six blocks from scratch is a hopeless pursuit because initially, the agent acts randomly in the hope of achieving high reward at least a few times. These rewards are used to reinforce actions leading to them. However, it is implausible that the agent will stack six blocks by executing a sequence of random actions. Due to a lack of success, the agent will not receive any learning signal (i.e., rewards) to update its policy. The policy will, therefore, remain random, and the agent will fail to learn the task. 
